VibrantLeaves: A principled parametric image generator for training deep restoration models

In this paper, we introduce a synthetic image generator relying on a few simple principles, specifically focusing on geometric modeling, textures, and a simple modeling of image acquisition. These principles, integrated into the classical Dead Leaves model, allow for the creation of high-quality training sets for image restoration tasks. Standard image denoising and super-resolution networks trained on these datasets achieve performance comparable to those trained on natural image datasets. The motivation behind this approach stems from the limitations of Deep Neural Networks in image restoration tasks. Despite their impressive performance, these networks are often poorly understood and prone to biases inherited from standard natural image training sets. To mitigate these issues, we emphasize the need for a better control over training sets, particularly through the use of synthetic and abstract datasets. Furthermore, our work includes a detailed analysis of the principles considered, identifying which image properties are necessary for maintaining high performance, thus taking a first step towards explainability. Besides, we show that neural networks trained with our synthetic sets naturally inherit robustness to the invariance properties of these sets, namely rotation and scale.

==> source/depth_of_field.tex <==
\renewcommand{\imageOneWidth}{2.5cm}

\begin{figure}
    \centering
    \begin{tikzpicture}
        % Définir les positions des images
        \node[anchor=west,inner sep=0] (img1) at (0,0) {\includegraphics[width=\imageOneWidth]{images/depth/background.png}};
        \node[anchor=west,inner sep=0] (img2) at ([xshift=0.5cm, yshift=0]img1.east) {\includegraphics[width=\imageOneWidth]{images/depth/midground.png}};
        \node[anchor=west,inner sep=0] (img3) at ([xshift=0.5cm, yshift=0]img2.east) {\includegraphics[width=\imageOneWidth]{images/depth/foreground.png}};
        \node[anchor=north,inner sep=0] (img4) at ([xshift=0cm, yshift=-0.5cm]img2.south) {\includegraphics[width=\imageOneWidth]{images/depth/fused.png}};
    
        % % Dessiner les flèches courbes
        \draw[->, thick] (img1) to[out=-90,in=180] node[midway, left]{$*B_{\sigma_1}$} (img4);
        \draw[->, thick] (img2) to[out=-90,in=90] (img4);
        \draw[->, thick] (img3) to[out=-90,in=0] node[midway, right]{$*B_{\sigma_2}$} (img4);

    \end{tikzpicture}
    \caption{Depth of field formation}
    \label{fig:depth_of_field}
\end{figure}




   % \node[anchor=south west,inner sep=0] (image0) at (-\imageOneWidth-1cm,-1cm) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch_teaser1.png}};
   %  \node[text width=4cm] at ([xshift=0, yshift=0.2cm]image0.north){\small Original / Noisy $(\sigma = 50)$};
    
   %  \node[anchor=south west,inner sep=0] (image1) at (\imageOneX,\imageOneY) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch_dl_1.png}};
   %  \node[text width=4cm] at ([xshift=0, yshift=0.2cm]image1.north){\small DRUNet-DL \cite{achddou_cviu}};


==> source/figure1.tex <==
% Changer la valeur de certaines variables
\renewcommand{\imageOneX}{0}
\renewcommand{\imageOneY}{0}
\renewcommand{\imageOneWidth}{4cm}


\renewcommand{\imageTwoXShift}{0}
\renewcommand{\imageTwoYShift}{-0.1\textwidth}
\renewcommand{\imageTwoWidth}{0.12\textwidth}
\renewcommand{\rectangleX}{1.2}
\renewcommand{\rectangleY}{1.2}

% \renewcommand{\rightCrop}{230}
% \renewcommand{\leftCrop}{300}
% \renewcommand{\upCrop}{150}
% \renewcommand{\bottomCrop}{150}

% \renewcommand{\rectangleX}{\imageOneWidth*0.299}
% \renewcommand{\rectangleY}{\imageOneWidth*(\bottomCrop*)}

% \renewcommand{\rectangleWidth}{\imageOneWidth*(768-\leftCrop -\rightCrop)/768}
% \renewcommand{\rectangleHeight}{\imageOneWidth*(512-\upCrop -\bottomCrop)/768}

\renewcommand{\rectangleWidth}{0.8}
\renewcommand{\rectangleHeight}{0.8}

\begin{figure*}[htp]
    \centering
    
    % \includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch.png}
    % \hfill
\begin{tikzpicture}
    % Charger la première image et la placer à une position spécifique
    \node[anchor=south west,inner sep=0] (image0) at (-\imageOneWidth-1cm,-1cm) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch_teaser1.png}};
    \node[text width=4cm] at ([xshift=0, yshift=0.2cm]image0.north){\small Original / Noisy $(\sigma = 50)$};
    
    \node[anchor=south west,inner sep=0] (image1) at (\imageOneX,\imageOneY) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch_dl_1.png}};
    \node[text width=4cm] at ([xshift=0, yshift=0.2cm]image1.north){\small DRUNet-DL \cite{achddou_cviu}};

    % Calculer la position du deuxième nœud en fonction de la position du premier nœud
    
    % \node[anchor=south,inner sep=0] (image2) at ([xshift=\imageTwoXShift, yshift=\imageTwoYShift]image1.south) {\includegraphics[width=\imageTwoWidth]{images/teaser_images/orig/monarch_dl_1.png}};
    
    % Calculer la position du deuxième nœud en fonction de la position du premier nœud
    \node[anchor=south,inner sep=0] (image2) at ([xshift=\imageTwoXShift, yshift=\imageTwoYShift]image1.south) {\includegraphics[width=\imageTwoWidth]{images/teaser_images/crops/monarch_dl_1.png}};

    % \node[anchor=south,inner sep=0] (image2) at ([xshift=\imageTwoXShift, yshift=\imageTwoYShift]image1.south) {\includegraphics[width=\imageTwoWidth,trim={230 150 300 150},clip]{images/teaser_images/orig/monarch_dl_1.png}};

    %Dessiner un carré vide à bords rouges sur la première image
    \draw[red, thick] (\rectangleX,\rectangleY) rectangle (\rectangleX+\rectangleWidth, \rectangleY+\rectangleHeight) ;

    % Relier le carré à l'autre image avec deux lignes en pointillés
    \draw[dashed, thick,red] (\rectangleX , \rectangleY ) -- (image2.north west);
    
    \draw[dashed, thick, red] (\rectangleX+\rectangleWidth , \rectangleY ) -- (image2.north east);
    \draw[red, thick] (image2.south east) rectangle (image2.north west) ;
\end{tikzpicture}
\begin{tikzpicture}
    % Charger la première image et la placer à une position spécifique
    \node[anchor=south west,inner sep=0] (image1) at (\imageOneX,\imageOneY) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch_dl_up.png}};
    \node[text width=4cm] at ([xshift=0, yshift=0.2cm]image1.north){\small \textbf{DRUNet-VL(Ours)}};

    % Calculer la position du deuxième nœud en fonction de la position du premier nœud
    \node[anchor=south,inner sep=0] (image2) at ([xshift=\imageTwoXShift, yshift=\imageTwoYShift]image1.south) {\includegraphics[width=\imageTwoWidth]{images/teaser_images/crops/monarch_dl_up.png}};

    % Dessiner un carré vide à bords rouges sur la première image
    \draw[red, thick] (\rectangleX,\rectangleY) rectangle (\rectangleX+\rectangleWidth, \rectangleY+\rectangleHeight) ;

    % Relier le carré à l'autre image avec deux lignes en pointillés
    \draw[dashed, thick,red] (\rectangleX , \rectangleY ) -- (image2.north west);
    
    \draw[dashed, thick, red] (\rectangleX+\rectangleWidth , \rectangleY ) -- (image2.north east);
    \draw[red, thick] (image2.south east) rectangle (image2.north west) ;
\end{tikzpicture}
\begin{tikzpicture}
    % Charger la première image et la placer à une position spécifique
    \node[anchor=south west,inner sep=0] (image1) at (\imageOneX,\imageOneY) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch_nat.png}};
    \node[text width=4cm] at ([xshift=0, yshift=0.2cm]image1.north){\small DRUNet-Nat \cite{zhang2021plug}};
    % Calculer la position du deuxième nœud en fonction de la position du premier nœud
    \node[anchor=south,inner sep=0] (image2) at ([xshift=\imageTwoXShift, yshift=\imageTwoYShift]image1.south) {\includegraphics[width=\imageTwoWidth]{images/teaser_images/crops/monarch_nat.png}};

    % Dessiner un carré vide à bords rouges sur la première image
    \draw[red, thick] (\rectangleX,\rectangleY) rectangle (\rectangleX+\rectangleWidth, \rectangleY+\rectangleHeight) ;

    % Relier le carré à l'autre image avec deux lignes en pointillés
    \draw[dashed, thick,red] (\rectangleX , \rectangleY ) -- (image2.north west);
    
    \draw[dashed, thick, red] (\rectangleX+\rectangleWidth , \rectangleY ) -- (image2.north east);
    \draw[red, thick] (image2.south east) rectangle (image2.north west) ;
\end{tikzpicture}


    \caption{Comparison of denoising results on the \textit{"Monarch.png"} image from Set14. The denoised images are the output of different versions of DRUNet\cite{zhang2021plug} trained on either Dead Leaves, VibrantLeaves or Natural Images.
    Our synthetic training, $\text{DRUNet}_{\text{VL}}$, achieves better image fidelity than DRUNet-DL, with and better detail preservation and less visual artifacts. (Best viewed on a digital screen)}
    \label{fig:teaser}
\end{figure*}



% \begin{tikzpicture}
%     % Charger la première image et la placer à une position spécifique
%     \node[anchor=south west,inner sep=0] (image1) at (\imageOneX,\imageOneY) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch.png}};

%     % Calculer la position du deuxième nœud en fonction de la position du premier nœud
%     \node[anchor=south,inner sep=0] (image2) at ([xshift=\imageTwoXShift, yshift=\imageTwoYShift]image1.south) {\includegraphics[width=\imageTwoWidth]{images/teaser_images/crops/monarch.png}};

%     % Dessiner un carré vide à bords rouges sur la première image
%     \draw[red, thick] (\rectangleX,\rectangleY) rectangle (\rectangleX+\rectangleWidth, \rectangleY+\rectangleHeight) ;

%     % Relier le carré à l'autre image avec deux lignes en pointillés
%     \draw[dashed, thick,red] (\rectangleX , \rectangleY ) -- (image2.north west);
    
%     \draw[dashed, thick, red] (\rectangleX+\rectangleWidth , \rectangleY ) -- (image2.north east);
%     \draw[red, thick] (image2.south east) rectangle (image2.north west) ;
% \end{tikzpicture}






% \begin{tikzpicture}    
%     \node[anchor=south west,inner sep=0] (image1) at (\imageOneX,\imageOneY) {\includegraphics[width=\imageOneWidth]{images/teaser_images/orig/monarch_dl_1.png}};
%     \node[anchor=south,inner sep=0] (image2) at ([xshift=\imageTwoXShift, yshift=\imageTwoYShift]image1.south) {\includegraphics[width=\imageOneWidth,trim={200 150 200 150},clip]{images/teaser_images/orig/monarch_dl_1.png}};
% \end{tikzpicture}
